Parameter estimation with the current generation of phenomenological waveform models applied to the black hole mergers of GWTC-1

We consider the ten confidently detected gravitational-wave signals in the GWTC-1 catalog which are consistent with mergers of binary black hole systems, and perform a thorough parameter estimation re-analysis. This is made possible by using computationally efficient waveform models of the current (fourth) generation of the IMRPhenom family of phenomenological waveform models, which consists of the IMRPhenomX frequency-domain modelsand the IMRPhenomT time-domain models. The analysis is performed with both precessing and non-precessing waveform models with and without subdominant spherical harmonic modes. Results for all events are validated with convergence tests, discussing in particular the events GW170729 and GW151226. For the latter and the other two lowest-mass events, we also compare results between two independent sampling codes, Bilby and LALInference. We find overall consistent results with the original GWTC-1 results, with all Jensen-Shannon divergences between the previous results using IMRPhenomPv2 and our default IMRPhenomXPHM posteriors below 0.045 bits, but we also discuss cases where including subdominant harmonics and/or precession influences the posteriors.

==> Preamble.tex <==
%auto-ignore

\makeatletter

%% Smaller space between section number and name
\def\@seccntformat#1{\csname the#1\endcsname.~}%

%% Smaller space between preceding text and new section headings
\def\section{%
  \@startsection {section}
  {1} {\z@} {0.55cm \@plus1ex \@minus .02ex}%
    {0.225cm} { \normalfont\bfseries \centering}%
}%
\def\subsection{%
  \@startsection {subsection}
  {2} {\z@ } {0.45cm \@plus 0.8ex \@minus 0.2ex}%
  {0.1125cm}{\normalfont \bfseries \centering }}
\def\subsubsection{%
  \@startsection {subsubsection}
  {3} {\z@ } {0.4cm \@plus 0.6ex \@minus 0.1ex}%
  {0.075cm}{\normalfont \it \centering }}

%% Headers and footers
\newcommand{\surnames}[1]{\def\@surnamelist{#1}\relax}
\surnames{\ }
\ifx \@shorttitle \@empty
  % \def\@oddhead{\small \MakeUppercase{\@title} \hfill}
  % Do nothing
\else
  \def\@oddhead{\small \MakeUppercase{\@shorttitle} \hfill}
\fi
\ifx \@surnamelist \@empty
  % Do nothing
\else
  \def\@evenhead{\small \MakeUppercase{\@surnamelist} \hfill}
\fi
\def\@oddfoot{\reset@font\hfil\thepage\hfil}%
\def\@evenfoot{\reset@font\hfil\thepage\hfil}%
\g@addto@macro\maketitle{\global\@specialpagetrue\gdef\@specialstyle{plain}}

%% Less hyphenation
\hyphenpenalty=1000  % Default: 50
%\tolerance=9000      % Default: 9999

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% This is all for the hyperref package and nice colors

%% The following conflicts with \texorpdfstring in section headers
% %% First, patch a bug from revtex4 to allow use of \nameref
% \usepackage{xpatch}% http://ctan.org/pkg/xpatch
% \makeatletter
% \xpatchcmd{\@ssect@ltx}{\@xsect}%
%   {\edef\@currentlabelname{#8}\@xsect}{}{}% Patch \<section>*
% \xpatchcmd{\@sect@ltx}{\@xsect}%
%   {\edef\@currentlabelname{#8}\@xsect}{}{}% Patch \<section>
% \makeatother

\definecolor{dodgerblue}{rgb}{0.12, 0.56, 1.0}
\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{alizarincrimson}{rgb}{0.82, 0.1, 0.26}
\definecolor{mediumpurple}{rgb}{0.58, 0.44, 0.86}
\definecolor{lasallegreen}{rgb}{0.03, 0.47, 0.19}
\definecolor{my_gray}{rgb}{0,0,0}
\definecolor{uniwienblue}{HTML}{006699}
\definecolor{walesred}{HTML}{ff0038}
\definecolor{myorange}{HTML}{FF6C0C}
\definecolor{ferngreen}{HTML}{009246}
\definecolor{scarletred}{HTML}{CD212A}

\usepackage[colorlinks, plainpages=false,
hyperfigures=true]{hyperref}
% \usepackage[pagebackref=true, colorlinks, plainpages=false,
% hyperfigures=true]{hyperref}
% \renewcommand*{\backref}[1]{}
% \renewcommand*{\backrefalt}[4]{%
%   \ifcase #1 \or (Cited on p.~#2.) \else %
%   (Cited on pp.~#2.) \fi %
% }
\hypersetup{linkcolor=dodgerblue}
\hypersetup{citecolor=CiteColor}
\hypersetup{urlcolor=dodgerblue}
\hypersetup{setpagesize=false}
% \hypersetup{unicode} % Clashes with '\G' command defined in Macros
\hypersetup{pdfborder=0 0 0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\makeatother

%\numberwithin{equation}{section}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> UsePackages.tex <==
%auto-ignore

%% Basic font packages
\newcommand{\hmmax}{0}
\newcommand{\bmmax}{0}
\usepackage[T3,T1]{fontenc}
%\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it} % For \mathpzc fonts
\usepackage{mathrsfs} % For \mathscr fonts
\usepackage{bm} % For \bm fonts
\makeatletter
\@ifclassloaded{beamer}
  { % if this is a beamer document, use sans-serif fonts
    \typeout{UsePackages: Detected beamer}
    \usepackage{tgheros}
    \renewcommand*\familydefault{\sfdefault}
  }
  { % otherwise:
    \typeout{UsePackages: Did not detect beamer}
    \ifx\asybeamer\undefined % use times for articles
    \typeout{UsePackages: Detected article}
    \usepackage[varg]{txfonts} % For math
    \usepackage{tgtermes} % For text
    \else % use beamer fonts for asy documents with beamer
    \typeout{Fonts: Detected asy for beamer}
    \usepackage{tgheros}
    \renewcommand*\familydefault{\sfdefault}
    \fi
  }
\usepackage{microtype} % For nicer alignment of text
\def\MT@register@subst@font{
  \MT@exp@one@n\MT@in@clist\font@name\MT@font@list
  \ifMT@inlist@\else\xdef\MT@font@list{\MT@font@list\font@name,}\fi}
\makeatother

% %% Compact the text (smaller intra-word spacing)
% \AtBeginDocument{
%   \setlength{\spaceskip}
%   {0.875\fontdimen2\font
%     plus 0.925\fontdimen3\font
%     minus 1\fontdimen4\font}
% }

%% Spread out the text lines slightly
\linespread{1.0425}

%% No extra space after periods
%\frenchspacing

%% A few necessary packages
\usepackage{graphicx} %
\usepackage[x11names,svgnames,rgb]{xcolor} %
% \usepackage[all]{onlyamsmath} % Error on bad non-ams math
\usepackage{xspace}
%% And a few optional ones
\usepackage{braket}
\usepackage{accents}
%\usepackage{rotating} % 'sidewaystable' support
\usepackage{siunitx}
\usepackage{mathtools}
\DeclareSymbolFontAlphabet{\mathrm}{operators}

%% Define a few colors
\definecolor{CiteColor}{rgb}{0.18039, 0.18824, 0.57255}
%\definecolor{CiteColor}{rgb}{0.250, 0.250, 0.800}
\definecolor{UrlColor} {rgb}{0.741, 0.173, 0.000}
\definecolor{DarkUrlColor} {rgb}{0.500, 0.110, 0.000}
\definecolor{LinkColor}{rgb}{0.25098, 0.47843, 0.04706}
%\definecolor{LinkColor}{rgb}{0.000, 0.502, 0.118}


%% To get the current font parameters and linewidth in a LaTeX
%% document, put \ShowFont at the appropriate place.  The results will
%% be printed in the log file (and/or to screen).
\makeatletter %
\newcommand{\ShowFont}{%
  \typeout{The main font is \f@encoding \space \f@family \space %
    \f@series \space \f@shape \space at \f@size pt.}%
  \typeout{The math font sizes are \tf@size pt (main), \sf@size pt %
    (script), and \ssf@size pt (scriptscript).}%
  \typeout{The linewidth is \the\linewidth}} %
\makeatother %
%% See the LaTeX2e font selection guide for more details.
%% Note also that captions in revtex4 are typeset with \small; when
%%   most of the document is 10pt, \small is 9pt.
%% In beamer, the default font is cmss and the math font size 10.95pt.
%% In revtex4, we have the following widths:
%%            onecolumn   twocolumn
%%     10pt     510pt       246pt
%%     12pt     468pt       229pt
%% PRD editors resize things to fit in a 200x200pt box by default, but
%%   I like to keep figures bigger.


\usepackage{xargs}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

